Evaluating 5G Networks for U-Space Applications: Insights from Dense Urban Measurement Campaign

Following the burgeoning interest in unmanned aerial vehicles (UAVs) utilization within human-inhabited spaces, critical challenges arise in ensuring reliable, low-latency communication-particularly important given the safety-critical nature of such operations in densely populated urban environments. Therefore, adequate cellular communication capabilities are essential to enable safe and effective operations within the so-called U-Spaces. In this context, this paper investigates the communication performance of cellular-connected UAVs in dense urban environments. In particular, the analysis is based on a comprehensive measurement campaign conducted in the city of Benidorm, Spain-an urban area well known for its high concentration of tall buildings and overall urban density. More specifically, we evaluated key performance indicators (KPIs) related to received signal strength and quality, data rate, and latency across various altitudes, mobile network operators, access technologies, and frequency bands, using multiple types of measurement equipment. The results highlight significant challenges, primarily due to the lack of dedicated planning for aerial coverage and interference management, revealing that current cellular networks may fall short in supporting reliable and ubiquitous UAVs communication. Thus, this paper calls for improved network solutions to ensure the reliability of UAV operations in urban airspace, thereby contributing to the integration of UAVs into urban logistics and mobility.

==> Figures/Figure_Results_Editor/RSRP_SINR_VerticalFlight_Scanner.tex <==
% \begin{figure*}[!t]
% \captionsetup[subfloat]{labelformat=empty}
%     % First row
%     \subfloat[\hspace{1.75cm}\footnotesize{(a) \ac{RSRP}}\label{subfig:Qualipoc_RSRP}]{
%         \setlength\fwidth{0.975\textwidth}
%         \setlength\fheight{0.25\textwidth}
%         \input{Figures/Tikz/BarPlot_Template_RSRP}
%     }
%     \\[0.5em] % Break to new row with extra vertical space

%     % Second row
%     \subfloat [\hspace{1.75cm}\footnotesize{(b) \ac{SINR}}\label{subfig:Qualipoc_SINR}]{
%         \setlength\fwidth{0.975\textwidth}
%         \setlength\fheight{0.25\textwidth}
%         \input{Figures/Tikz/BarPlot_Template_SINR}
%     }

%     \caption{Mean measured \ac{RSRP} (Fig. xxx) and \ac{SINR} (Fig. xxx) by the TSMA6B scanner during the hovering vertical flight
% at different altitudes and frequency bands.\label{fig:xxx}}
% \end{figure*}


\begin{figure*}[!t]
\captionsetup[subfloat]{labelformat=empty}
    % First row
    \subfloat[\footnotesize{(a) \ac{RSRP}}\label{subfig:VertFlight_RSRP_LTE_NR}]{
        \setlength\fwidth{0.975\columnwidth}
        \setlength\fheight{0.6026\columnwidth}
        \input{Figures/Tikz/TEST}
    }
    % \\[0.5em] % Break to new row with extra vertical space
    %
    % Second row
    \subfloat [\footnotesize{(b) \ac{SINR}}\label{subfig:VertFlight_SINR_LTE_NR}]{
        \setlength\fwidth{0.975\columnwidth}
        \setlength\fheight{0.6026\columnwidth}
        \input{Figures/Tikz/TEST}
    }

    \caption{Mean measured \ac{RSRP} (Fig.~\ref{subfig:VertFlight_RSRP_LTE_NR}) and \ac{SINR} (Fig.~\ref{subfig:VertFlight_SINR_LTE_NR}) by the TSMA6B scanner during the hovering vertical flight
at different altitudes and frequency bands.\label{fig:VertFlight_RSRP_SINR_LTE_NR}}
\end{figure*}



==> Sections/04_Measurement_campaign.tex <==
% \section{Measurement Campaign}
% \label{sec:measurement_campign}

% The measurement campaign was structured into %three 
% {\color{blue}two} types of experiments: 
% horizontal flights and ground drive tests. %, vertical flights,
% % Each type of test captured data on coverage and signal quality at different heights and locations, 
% % providing a comprehensive view of the \ac{LTE} and \ac{NR} networks.

% \subsubsection{Horizontal UAV Flights}
% \label{subsec:MeasurementCapaign_HorFlight}

% % The horizontal flights at various heights where performed in both Block\,1 and Block\,2, 
% % respectively shown in green and in red in Fig.~\ref{fig:MeasurementArea}. 
% % In each block, 
% % the drone followed a dense, squared grid pattern to map coverage within each area.
% % The flights were conducted at altitudes of 20\,m, 40\,m, and the upper limit of 60\,m,
% % with the \ac{UAV} moving at a speed of 4\,m/s.
% % Each flight lasted 6-7 minutes, 
% % with a total of six flights across the two blocks and altitudes. 
% % Start and end times were recorded to maintain measurement consistency, 
% % enabling direct comparisons between scanner and phone data. 
% {\color{blue}
% Horizontal flights were performed at heights of 20 m, 40 m and 60 m, complying with the height limit for flight allowed in urban environments, and were performed in both Block 1 and Block 2, as shown in Fig. \ref{fig:MeasurementArea}. In each block; the drone followed a dense, gridded flight pattern to map the coverage within each zone. The tests were conducted at the speed of 4 m/s for both blocks; additionally, for block 1, the survey was conducted at 8 m/s; therefore, each flight lasted between 6 and 10 minutes. Finally, to maintain the consistency of the measurements, the start and end times were recorded, allowing direct comparisons between the scanner and telephone data.}
% % \subsubsection{Vertical Flights}
% % \label{subsec:MeasurementCapaign_VerFlight}

% % \red{Vertical flights were conducted at a specific point within Block 1, 
% % chosen to ensure \ac{LoS} with a nearby \ac{BS} on a tall building. 
% % The drone ascended incrementally to altitudes of 10\,m, 20\,m, 30\,m, 40\,m, 50\,m, and 60\,m.
% % At each altitude, 
% % signals were sampled for one minute to collect representative data.
% % No data was collected when the drone descended. }

% \subsubsection{Ground Drive Tests}
% \label{subsec:groundDriveTest}

% % A ground drive test was conducted with a vehicle traversing the streets surrounding the measurement area. 
% % The antenna, 
% % positioned 1\,m above the ground, 
% % simulated a mobile device in motion. 
% % The 25-minute route provided comprehensive signal coverage mapping while on the move, 
% % revealing variations in signal quality due to continuous movement within the cluster of buildings in the urban environment. 
% % The sampling configuration was consistent with that of the aerial tests, 
% % enabling a direct comparison with aerial measurements, 
% % and facilitating a comprehensive assessment of potential \ac{UAV} performance in comparison to today’s \ac{gUE}.
% {\color{blue}
% A ground drive test was conducted with a vehicle with an average duration of 25 minutes around the measurement area. The antenna was mounted at a height of 1 m, simulating a moving mobile device. The sampling parameters matched those used in the aerial tests, allowing a direct comparison. This configuration allowed mapping of signal variations caused by continuous movement through dense urban structures, providing a baseline to assess the performance of UAVs compared to the \ac{gUE}.}


==> Tables/RSRP_Scanner_Stats.tex <==
\begin{table}[!b]
%\vspace{-1em}
\centering
\begin{tabular}{l l c c c c}
\hline
 % & & \multicolumn{4}{c|}{\textbf{RSRP [dBm]}} \\
\textbf{Frequency Band}              &  & \textbf{gUE} & \textbf{20\,m} & \textbf{40\,m} & \textbf{60\,m} \\ \hline
\multirow{2}{*}{\textbf{B3 (LTE)}} & 5\%-Tile  & -104.9       & -91.5         & -93.7         & -95.8         \\ %\cline{2-6} 
                                     & Median     & -96.3        & -83.8         & -86.4         & -86.9         \\ %\cline{2-6} 
                                     & Mean       & -94.2        & -83           & -85.7         & -87.2         \\ \hline
\multirow{2}{*}{\textbf{n78 (NR)}}  & 5\%-Tile & -97.6        & -88.3         & -91.4         & -90.9         \\ %\cline{2-6} 
                                     & Median     & -86.2        & -79.3         & -80           & -81.1         \\ %\cline{2-6} 
                                     & Mean       & -85.3        & -78.2         & -79.9         & -80.9         \\ \hline
\end{tabular}
\vspace{0.5em}
\caption{Summary of obtained TSMA6B scanner \ac{RSRP} statistics.
\label{tab:Statistic_Scanner_RSRP}}
% \vspace{-3em}
\end{table}


==> Tables/SINR_Scanner_Stats.tex <==

\begin{table}[!t]
% \vspace{0.22cm}
\centering
\begin{tabular}{l l c c c c}
\hline
% & & \multicolumn{4}{c|}{\textbf{SINR [dB]}} \\
\textbf{Frequency Band}                                                     &  & \textbf{gUE} & \textbf{20\,m} & \textbf{40\,m} & \textbf{60\,m} \\ \hline
\multirow{2}{*}{\textbf{TSMA6B B3 (LTE)}} & 5\% Tile  & -7.1         & -8            & -9.4          & -10.5         \\ %\cline{2-6} 
                                         & Median     & 6            & 3.4           & 1.3           & -5.6          \\ %\cline{2-6} 
                                         & Mean       & 5.6          & 3             & -0.6          & -4.2          \\ %\hline
\multirow{2}{*}{\textbf{TSMA6B n78 (NR)}}  & 5\% Tile  & 1.1          & -4            & -7.6          & -7.2          \\ %\cline{2-6} 
                                         & Median     & 11.7         & 7.5           & 5.7           & 4.1           \\ %\cline{2-6} 
                                         & Mean       & 11.8         & 7.5           & 5.4           & 3.6           \\ \hline
% \multirow{2}{*}{\textbf{QualiPoc Phone}}  
% & 5\% Tile   & -1.4           & -2.7           & -6.8           & -8.5           \\ 
% & Median     & 12.7          & 7.5             & 3.9            & 3.0            \\ 
% & Mean       & 12.7          & 7.5             & 4.0            & 3.1            \\ \hline

\end{tabular}
\vspace{0.5em}
\caption{Summary of \ac{SINR} statistics for TSMA6B and Qaulipoc phone.
\label{tab:Statistic_Scanner_SINR}}
\vspace{-3em}
\end{table}


==> Tables/Thp_Scanner_Stats.tex <==
\begin{table}[!t]
% \vspace{0.22cm}
\centering
\begin{tabular}{l l c c c c}
\hline

\textbf{Frequency Band}   &  & \textbf{gUE} & \textbf{20\,m} & \textbf{40\,m} & \textbf{60\,m} \\ \hline

\multirow{2}{*}{\textbf{Thp DL [Mbps] }}  
& 5\% Tile  & 10.80          & 10.96           & 9.21           & 9.71           \\ 
& Median    & 105.65         & 99.60           & 41.45          & 66.0            \\ 
& Mean      & 110.18         & 140.65          & 88.73          & 95.34            \\ \hline


\multirow{2}{*}{\textbf{RTT [ms] }}  
& 5\% Tile  & 42.74          & 53.57           & 54.50          & 53.42           \\ 
& Median    & 54.0           & 55.90           & 58.03          & 59.91            \\ 
& Mean      & 62.09          & 58.65           & 59.98          & 66.41            \\ \hline



\end{tabular}
\vspace{0.5em}
\caption{Summary of Qualipoc phone throughput and \ac{RTT} statistics.
\red{[Matteo]: In the text before you wrote, regarding the iPerf3 setup that is for UL and DL. However here there is only DL. Do we have UL has well? }
\label{tab:Statistic_Thp_RTT}}
\vspace{-2.5em}
\end{table}
